Bearing-Based Formation Control with Optimal Motion Trajectory

Bearing-based distributed formation control is attractive because it can be implemented using vision-based measurements to achieve a desired formation. Gradient-descent-based controllers using bearing measurements have been shown to have many beneficial characteristics, such as global convergence, applicability to different graph topologies and workspaces of arbitrary dimension, and some flexibility in the choice of the cost. In practice, however, such controllers typically yield convoluted paths from their initial location to the final position in the formation. In this paper we propose a novel procedure to optimize gradient-descent-based bearing-based formation controllers to obtain shorter paths. Our approach is based on the parameterization of the cost function and, by extension, of the controller. We form and solve a nonlinear optimization problem with the sum of path lengths of the agent trajectories as the objective and subject to the original equilibria and global convergence conditions for formation control. Our simulation shows that the parameters can be optimized from a very small number of training samples (1 to 7) to straighten the trajectory by around 16% for a large number of random initial conditions for bearing-only formation. However, in the absence of any range information, the scale of the formation is not fixed and this optimization may lead to an undesired compression of the formation size. Including range measurements avoids this issue and leads to further trajectories straightening by 66%.

==> preamble/compactLists.tex <==
% set compact lists
\setlist[1]{\labelindent=\parindent}
\setlist[1]{topsep=3pt, itemsep=0pt}


==> preamble/courseFormatting.tex <==
%make underscore work without escaping in text mode
\usepackage{underscore}

%Common style that will be used for titles
\newcommand{\titlestyle}{\color{DodgerBlue3}\sffamily}

%Perfect 1-inch margins
\usepackage[margin=1in]{geometry}
\usepackage[medium,compact]{titlesec}
\usepackage{longtable}
\titleformat*{\section}{\titlestyle \Large}
\titleformat*{\subsection}{\titlestyle \large \itshape}

%Lists (requires enumitem package):
%Font for description
\setlist[description]{font=\color{DodgerBlue3}}
%Compact lists
\setlist[1]{\labelindent=\parindent}
\setlist[1]{topsep=3pt, itemsep=0pt}

%Format main title
\let\prevtitle\title
\renewcommand{\title}[1]{\prevtitle{\titlestyle #1}}
\let\prevauthor\author
\renewcommand{\author}[1]{\prevauthor{\titlestyle #1}}
\let\prevdate\date
\renewcommand{\date}[1]{\prevdate{\titlestyle #1}}

%Displayed quotations (used to define an environment for function specification)
\usepackage{csquotes}


%Include code
\usepackage{listings}

%formatting for the description of a function's input/output arguments
\mdfdefinestyle{functionspecification}{%
linecolor=DodgerBlue3,
rightline=false, topline=false, bottomline=false,
outerlinewidth=1.35,
roundcorner=10pt,
innerleftmargin=1.2em,
innertopmargin=0.3em,
innerbottommargin=0.3em,
leftmargin=1pt,
skipabove=0.5em,  
skipbelow=0.5em,  
backgroundcolor=white}

\newcommand{\dstar}{$\bigstar$}


==> preamble/courseProblemSet.tex <==
\input{preamble/courseFormatting}

%Facilities for markers file
% open file the beginning of the document
\AtBeginDocument{%
  \newwrite\markerstream
  \immediate\openout\markerstream=\jobname.mlg
}
% close the file at the end of the document
\AtEndDocument{%
  \immediate\closeout\markerstream
}
%definition similar to \typeout, but for markers
\makeatletter
\newcommand{\markerout}[1]{\begingroup \set@display@protect \immediate \write \markerstream {#1}\endgroup}
\makeatother

\usetikzlibrary{intersections}

\titleformat{\section}{\titlestyle\large\bfseries}{Problem \thesection:}{0.5ex}{}
%\titleformat{\subsection}{\normalfont\bfseries}{Problem \thesubsection:}{0.5ex}{}
\titleformat{\paragraph}[runin]{\titlestyle\normalsize\bfseries}{}{2pt}{}

%Macro for paragraph header for preparation steps to questions
%\newcommand{\preparation}{\smallskip\par\noindent\textbf{\titlestyle Preparation.~}}

\newcommand{\preparation}[1][]{%
\smallskip\par\noindent%
\textbf{\titlestyle Preparation \displayifnotempty{~(}{#1}{)}.~}}

%New custom counter for question
\newcounter{question}[section]

%Macro for writing points for the current question to the log file.
\newcommand{\pointmarker}{\typeout{Question points marker [\thesection.\thequestion] [\questionpoints]}}

\makeatletter
%Makes questions that:
%- are automatically numbered using the format <sectionNumber>.<questionNumber>
%- can be referred to using the usual \label-\ref mechanism
%- if the optional argument is not empty, this is displayed in parenthesis (typically, this will be a \points{n} or a \optional command). If the optional argument is empty, a single point is silently added to the point counter.
\newcommand{\question}[1][]{%
\smallskip\par\noindent%
\refstepcounter{question}\zerovar{\questionpoints}%
\sbox\boxifnotempty{\textbf{\titlestyle #1}}% for some reason, if the box is saved inside the \textbf{\titlestyle ...} (to avoid repeating the style), the box counts as empty for \ifempty, so I need to repeat the style here.
\textbf{\titlestyle Question \thesection.\thequestion\displayifnotempty{~(}{\usebox{\boxifnotempty}}{)}.~}%
\ifempty{\usebox{\boxifnotempty}}{\increasepoints{1}}%
\def\@currentlabel{{\thesection.\thequestion}}\pointmarker}
\makeatother
\newcommand{\hintquestion}[1]{\paragraph{Hint
    for question \ref{#1}:~}}
\newcommand{\hint}{\paragraph{Hint:~}}

\newcommand{\answer}[1][]{\smallskip\leavevmode\\\noindent\textbf{Answer \thesection.\thequestion#1:~}}

\newcommand{\updated}[1]{{\color{red} #1}}

\newcolorlabel{labeloptional}{DodgerBlue3}
\newcommand{\optional}{\labeloptional{optional}}
\newcolorlabel{labelprovided}{Orange1}
\newcommand{\provided}{\labelprovided{provided}}
\newcolorlabel{labelvideo}{OliveDrab3}
\newcommand{\video}{\labelvideo{video}}
\newcolorlabel{labelimage}{DarkOrchid2}
\newcommand{\image}{\labelimage{image}}
\newcolorlabel{labelcode}{SlateBlue2}
\newcommand{\code}{\labelcode{code}}
\newcolorlabel{labelscan}{Chocolate3}
\newcommand{\scan}{\labelcode{scan}}
\newcolorlabel{labelnew}{OliveDrab3}
\newcommand{\lbnew}{\labelnew{new}}

%\newcommand{\optional}{{\titlestyle optional}}

\tikzset{point/.style={inner sep=0pt,fill=black,circle,minimum size=4pt}}

%macros for keeping track of points (total, and for current question)
\zerovar{\totalpoints}
\zerovar{\bonuspoints}
\zerovar{\questionpoints}
\newcommand{\increasepoints}[1]{\addtovar{\totalpoints}{#1}\addtovar{\questionpoints}{#1}}
\newcommand{\points}[1]{#1 point\ifthenelse{\equal{#1}{1}}{}{s}\increasepoints{#1}}
\makeatletter
\newcommand{\totalpointswithbonus}[1]{\pgfmathparse{\storeddef{totalpoints}+#1}\pgfmathresult\typeout{Total points marker [\pgfmathresult]}}
\makeatother

\newstoreddef{totalpoints} %remember total number of points in aux file

% answer boxes
\newcommand{\vspaceboxdelta}{3mm}
\newcommand{\vspacebox}[1]{\par\bigskip{\tikz{\useasboundingbox (0,-\vspaceboxdelta) rectangle (\textwidth,#1\baselineskip); \draw[gray!20!white,line width=3pt] (-\vspaceboxdelta,-\vspaceboxdelta) rectangle (\textwidth+2*\vspaceboxdelta,#1\baselineskip+\vspaceboxdelta);}}\par}
\newcommand{\vspaceoneline}{\vspacebox{2}}
\newcommand{\vspacetwolines}{\vspacebox{3}}
\newcommand{\vspacethreelines}{\vspacebox{4}}
\newcommand{\vspacefourlines}{\vspacebox{5}}

% text fields
\newcommand{\textrowfield}[1]{\par\noindent#1: \enspace\hrulefill}

% formatting for the description of a function's input/output arguments
\usepackage[framemethod=tikz]{mdframed}
\mdfdefinestyle{functionspecification}{%
linecolor=DodgerBlue3,
rightline=false, topline=false, bottomline=false,
outerlinewidth=1.35,
roundcorner=10pt,
innerleftmargin=1.2em,
innertopmargin=0.3em,
innerbottommargin=0.3em,
leftmargin=1pt,
skipabove=0.5em,  
skipbelow=0.5em,  
backgroundcolor=white}
\mdfdefinestyle{classspecification}{%
linecolor=DarkOliveGreen3,
rightline=false, topline=false, bottomline=false,
outerlinewidth=1.35,
roundcorner=10pt,
innerleftmargin=1.2em,
innertopmargin=0.3em,
innerbottommargin=0.3em,
leftmargin=1pt,
skipabove=0.5em,  
skipbelow=0.5em,  
backgroundcolor=white}
%Note: I was not able to avoid duplication of options.

\newenvironment{functionspecification}{\markerout{Marker function [start]}\begin{mdframed}[style=functionspecification]}
{\markerout{Marker function [end]}\end{mdframed}}%
\newenvironment{classspecification}{\markerout{Marker class [start]}\begin{mdframed}[style=classspecification]}
{\markerout{Marker class [end]}\end{mdframed}}%
%\NewEnviron{fdescription}{\par\noindent{\titlestyle Description}: \BODY\markerout{Marker text [description] [start]^^J\BODY^^JMarker text [description] [end]}\par}
\NewEnviron{fdescription}{\par\noindent{\titlestyle Description}: \BODY\markerout{Marker text [description] [start]^^J\BODY^^JMarker text [description] [end]}\par}
\newenvironment{cdescription}{\fdescription}{\endfdescription}
\NewEnviron{frequirements}{\par\noindent{\titlestyle Requirements}: \BODY\markerout{Marker text [requirements] [start]^^J\BODY^^JMarker text [requirements] [end]}\par}
\newcommand{\cname}[1]{\noindent{\titlestyle Class name}: \var{#1}\par}
\newenvironment{finputs}{\markerout{Marker argument_group [start] [inputs]}\noindent{\titlestyle Input arguments}\begin{itemize}}{\end{itemize}\markerout{Marker argument_group [end]}}
\newenvironment{foutputs}[1][Output]{\markerout{Marker argument_group [start] [outputs]}\noindent{\titlestyle #1 arguments}\begin{itemize}}{\end{itemize}\markerout{Marker argument_group [end]}}
\newcommand{\freturns}[2][]{\noindent{\titlestyle Returns}: \var{#2}\displayifnotempty{ (type }{\var{#1}}{)}}
\newcommand{\argument}[4][]{\markerout{Marker argument [start]}\markerout{Marker argument [name] [#2]}\var{#2} %
  \ifnotempty{#1#3}{(\ifnotempty{#3}{\markerout{Marker argument [dimensions] [#3] [#4]}dim. \vardim{#3}{#4}\ifnotempty{#1}{, }}%
  \displayifnotempty{\markerout{Marker argument [type] [#1]}type }{\var{#1}}{})}\markerout{Marker argument [end]}}
\newcommand{\argumentscalar}[2][]{\argument[#1]{#2}{}{}}
\newcommand{\fheader}[3][]{\noindent{\titlestyle Header}: \function[#1]{#2}{#3}\par}
\newcommand{\fname}[2][Function]{\noindent{\titlestyle #1 name}: \var{#2}\par}
\newcommand{\ffilename}[1]{\noindent{\titlestyle File name}: \file{#1}\par}
\newcommand{\functionheader}[3][]{\markerout{Marker function_header [#1] [#2] [#3]}\function[#1]{#2}{#3}\par}

%ROS node specification
\newenvironment{nodespecification}{\begin{mdframed}[style=functionspecification]%
\newcommand{\filename}[1]{\par{\titlestyle File name:} \file{##1}}
\renewenvironment{description}{\par\noindent{\titlestyle Description:}}{\par}%
\newenvironment{subscribers}{\par\noindent{\titlestyle Subscribes to topics:}}{}%
\newenvironment{publishers}{\par\noindent{\titlestyle Publishes to topics:}}{}%
%
}{\end{mdframed}}

\newcommand{\rostopic}[2]{\var{#1} (type \var{#2})}

% Macros for questions where student need to draw on axes
\newcommand{\drawingaxes}[1][]{\draw[gray] (-5,-5) grid (5,5);
  \draw[very thick, -latex] (-5.7,0) -- (5.7,0);
  \draw[very thick, -latex] (0,-5.7) -- (0,5.7); #1}
\newcommand{\shifteddrawingaxes}[1][]{
  \begin{scope}[xshift=15cm]
    \drawingaxes[#1]
  \end{scope}
}

\newcommand{\drawexercise}[2][]{\begin{center}
\begin{tikzpicture}[scale=0.6]
  \node[text width=5cm,anchor=west]{#2};
  \shifteddrawingaxes[#1]
\end{tikzpicture}
\end{center}
}


==> preamble/courseProblemSetSectionsLettered.tex <==
%Change format of numbering for questions to letters instead of numbering
\renewcommand{\thequestion}{\alph{question}}


==> preamble/courseSyllabus.tex <==
 \input{preamble/courseFormatting}


\newlength{\topicwidth}
\newlength{\topicdatewidth}
\setlength{\topicdatewidth}{19mm}
\newlength{\duewidth}
\setlength{\duewidth}{23mm}

%Create a topictable environment from the longtable environment
\newenvironment{topictable}[1][2cm]%
{\newcommand{\picswidth}{#1}\setlength{\topicwidth}{\textwidth-\picswidth-\topicdatewidth-\duewidth-12.5mm}%
\setcounter{topic}{1}\begin{longtable}{p{\picswidth}p{\topicwidth}p{\topicdatewidth}p{\duewidth}}}%
{\end{longtable}}

%Prepare counter and relative macros for handling array of class dates
\newcount\i
\pgfmathsetcount{\i}{0}
\def\classdate{\pgfprint{\classdatearray[\i]}\global\advance\i 1\relax}

%Counters for topic and subtopic
\newcounter{topic}
\newcounter{subtopic}

%Topichead
\def\topichead#1#2#3{\rowcolor{SlateGray1}{\setcounter{subtopic}{1}\rule{0pt}{16pt}\titlestyle Topic \arabic{topic}\addtocounter{topic}{1}} & \multicolumn{3}{l}{{\titlestyle #1:} #2 \rule[-8pt]{0pt}{12pt}}\\\tikz[overlay]{\node[anchor=north west,inner sep=0pt]{\includegraphics[width=\picswidth,keepaspectratio]{figures/#3}};}}
\def\firstsubtopic#1{ & \makecell[{{p{\topicwidth}}}]{\rule{0pt}{14pt}#1}\addtocounter{subtopic}{1}}
\def\subtopic#1{\\ \cmidrule{2-4} & \makecell[{{p{\topicwidth}}}]{#1}\addtocounter{subtopic}{1}}
%\def\topicdate#1{& \makecell[{{p{\topicdatewidth}}}]{#1}}
\newcommand{\topicdate}[1][\classdate]{& \makecell[{{p{\topicdatewidth}}}]{#1}}
\def\due#1{& \makecell[{{p{\duewidth}}}]{#1}}
\def\endtopic{\\}
\newcolorlabel{labelhw}{Orange1}
\newcommand{\hwdue}[1]{\labelhw{HW #1}}
\newcolorlabel{paperdue}{Tomato1}
\newcolorlabel{examdue}{Tomato1}
\newcolorlabel{labelMH}{DodgerBlue3}
\newcommand{\mhday}{\labelMH{M-H}~}
\newcolorlabel{labelqz}{Sienna3}
\newcommand{\qzdue}[1]{\labelqz{QZ #1}~}

%TODO: Add automatic test to check if a subtopic is the first subtopic, and adjust the formatting accordingly.
%The subtopic counter is already there, but due to conflicts with the tabular environment, I was not able to include the test inside the \subtopic macro.
%\def\tpctest{\noalign{\ifnum\value{subtopic}=1{}\else{\hrule}\fi}}


==> preamble/generateGraphLocalization <==
#!/usr/bin/env python
# Note: in the list of node and edge quantities: first element is the name to use in the command name,
# the second is the one to use in the definition

import os
f=open('graphLocalization.tex','w')

f.write('% This file was generated by the script'+os.path.basename(__file__)+'\n')
f.write('% Do not modify this file directly\n\n')

f.write('% Notation for nodes\n')
nodeIndexList=['i','j']
nodeStateDoubleList=[['R','R'],['T','T']]
for index in nodeIndexList:
    for state in nodeStateDoubleList:
        f.write('\\newcommand{\\'+state[0]+index+'}{'+state[1]+'_{'+index+'}}\n')
        f.write('\\newcommand{\\d'+state[0]+index+'}{\\dot{'+state[1]+'}_{'+index+'}}\n')
        f.write('\\newcommand{\\dd'+state[0]+index+'}{\\ddot{'+state[1]+'}_{'+index+'}}\n')
    f.write('\n')
f.write('\n')

edgeIndexList=['ij','ji']
edgeStateDoubleList=[['R','R'],['T','T'],['beta','\\beta'],['c','c'],['d','d'],['q','q'],['l','\\lambda'],['varphi','\\varphi'],['g','g']]

f.write('% Notation for edges\n')
for index in edgeIndexList:
    for state in edgeStateDoubleList:
        f.write('\\newcommand{\\'+state[0]+index+'}{'+state[1]+'_{'+index+'}}\n')
    f.write('\n')
f.write('\n')

f.write('% Notation for edges, measured quantities\n')
for index in edgeIndexList:
    for state in edgeStateDoubleList:
        f.write('\\newcommand{\\t'+state[0]+index+'}{\\tilde{'+state[1]+'}_{'+index+'}}\n')
        f.write('\\newcommand{\\dt'+state[0]+index+'}{\\dot{\\tilde{'+state[1]+'}}_{'+index+'}}\n')
    f.write('\n')
f.write('\n')

f.write('% Node state differences\n')
f.write('\\newcommand{\\xjmi}{x_j-x_i}\n')
f.write('\\newcommand{\\vjmi}{v_j-v_i}\n')
f.write('\\newcommand{\\nxjmi}{\\norm{\\xjmi}}\n')
f.write('\n')

f.write('% Notation for desired quantities\n')
quantityTripleList=[['x','x','i'],['x','x','j'],['beta','\\beta','ij'],['d','d','ij']]
for quantity in quantityTripleList:
    f.write('\\newcommand{\\'+quantity[0]+'g'+quantity[2]+'}{'+quantity[1]+'_{g,'+quantity[2]+'}}\n')

f.close()






        


==> preamble/generateNotation <==
#!/usr/bin/env python
import string
import os
f=open('notation.tex','w')

f.write('% This file was generated by the script'+os.path.basename(__file__)+'\n')
f.write('% Do not modify this file directly\n\n')

f.write('% Shortand notation for vectors and their derivatives\n')
for c in string.ascii_lowercase+string.ascii_uppercase:
    f.write('\\providecommand{\\v'+c+'}{\\vct{'+c+'}}\n')
    f.write('\\providecommand{\\dv'+c+'}{\\dot{\\vct{'+c+'}}}\n')
    f.write('\\providecommand{\\tv'+c+'}{\\tilde{\\vct{'+c+'}}}\n')
    f.write('\\providecommand{\\dtv'+c+'}{\\dot{\\tilde{\\vct{'+c+'}}}}\n')
f.write('\n')
for c in [['beta','\\beta'],['sigma','\\sigma']]:
    f.write('\\providecommand{\\v'+c[0]+'}{\\boldsymbol{'+c[1]+'}}\n')
    f.write('\\providecommand{\\dv'+c[0]+'}{\\dot{\\boldsymbol{'+c[1]+'}}}\n')
f.write('\n')
for c in ['e']:
    f.write('\\providecommand{\\t'+c+'}{\\tilde{'+c+'}}\n')
f.write('\n')

f.write('% Shortand notation for derivatives and bold of symbols\n')
for c in [['gamma','\\gamma'],['Delta','\Delta']]:
    f.write('\\providecommand{\\d'+c[0]+'}{\\dot{'+c[1]+'}}\n')
    f.write('\\providecommand{\\dd'+c[0]+'}{\\ddot{'+c[1]+'}}\n')
    f.write('\\providecommand{\\v'+c[0]+'}{\\bm{'+c[1]+'}}\n')
f.write('\n')


f.write('% Shortand notation for matrices\n')
for c in string.ascii_uppercase:
    f.write('\\providecommand{\\m'+c+'}{\\vct{'+c+'}}\n')
f.write('\n')

f.write('% Shortand notation for calligraphic upper case letters\n')
for c in string.ascii_uppercase:
    f.write('\\providecommand{\\c'+c+'}{\\mathcal{'+c+'}}\n')
f.write('\n')

f.write('% Shortand notation for some tilded symbols and their derivatives\n')
symbolDoubleList=[['x','x'],['y','y'],['varphi','\\varphi']]
for symbol in symbolDoubleList:
    f.write('\\providecommand{\\t'+symbol[0]+'}{\\tilde{'+symbol[1]+'}}\n')
    f.write('\\providecommand{\\dt'+symbol[0]+'}{\\dot{\\tilde{'+symbol[1]+'}}}\n')
f.write('\n')

f.close()


==> preamble/graphLocalization.tex <==
% This file was generated by the scriptgenerateGraphLocalization
% Do not modify this file directly

% Notation for nodes
\newcommand{\Ri}{R_{i}}
\newcommand{\dRi}{\dot{R}_{i}}
\newcommand{\ddRi}{\ddot{R}_{i}}
\newcommand{\Ti}{T_{i}}
\newcommand{\dTi}{\dot{T}_{i}}
\newcommand{\ddTi}{\ddot{T}_{i}}

\newcommand{\Rj}{R_{j}}
\newcommand{\dRj}{\dot{R}_{j}}
\newcommand{\ddRj}{\ddot{R}_{j}}
\newcommand{\Tj}{T_{j}}
\newcommand{\dTj}{\dot{T}_{j}}
\newcommand{\ddTj}{\ddot{T}_{j}}


% Notation for edges
\newcommand{\Rij}{R_{ij}}
\newcommand{\Tij}{T_{ij}}
\newcommand{\betaij}{\beta_{ij}}
\newcommand{\cij}{c_{ij}}
\newcommand{\dij}{d_{ij}}
\newcommand{\qij}{q_{ij}}
\newcommand{\lij}{\lambda_{ij}}
\newcommand{\varphiij}{\varphi_{ij}}
\newcommand{\gij}{g_{ij}}

\newcommand{\Rji}{R_{ji}}
\newcommand{\Tji}{T_{ji}}
\newcommand{\betaji}{\beta_{ji}}
\newcommand{\cji}{c_{ji}}
\newcommand{\dji}{d_{ji}}
\newcommand{\qji}{q_{ji}}
\newcommand{\lji}{\lambda_{ji}}
\newcommand{\varphiji}{\varphi_{ji}}
\newcommand{\gji}{g_{ji}}


% Notation for edges, measured quantities
\newcommand{\tRij}{\tilde{R}_{ij}}
\newcommand{\dtRij}{\dot{\tilde{R}}_{ij}}
\newcommand{\tTij}{\tilde{T}_{ij}}
\newcommand{\dtTij}{\dot{\tilde{T}}_{ij}}
\newcommand{\tbetaij}{\tilde{\beta}_{ij}}
\newcommand{\dtbetaij}{\dot{\tilde{\beta}}_{ij}}
\newcommand{\tcij}{\tilde{c}_{ij}}
\newcommand{\dtcij}{\dot{\tilde{c}}_{ij}}
\newcommand{\tdij}{\tilde{d}_{ij}}
\newcommand{\dtdij}{\dot{\tilde{d}}_{ij}}
\newcommand{\tqij}{\tilde{q}_{ij}}
\newcommand{\dtqij}{\dot{\tilde{q}}_{ij}}
\newcommand{\tlij}{\tilde{\lambda}_{ij}}
\newcommand{\dtlij}{\dot{\tilde{\lambda}}_{ij}}
\newcommand{\tvarphiij}{\tilde{\varphi}_{ij}}
\newcommand{\dtvarphiij}{\dot{\tilde{\varphi}}_{ij}}
\newcommand{\tgij}{\tilde{g}_{ij}}
\newcommand{\dtgij}{\dot{\tilde{g}}_{ij}}

\newcommand{\tRji}{\tilde{R}_{ji}}
\newcommand{\dtRji}{\dot{\tilde{R}}_{ji}}
\newcommand{\tTji}{\tilde{T}_{ji}}
\newcommand{\dtTji}{\dot{\tilde{T}}_{ji}}
\newcommand{\tbetaji}{\tilde{\beta}_{ji}}
\newcommand{\dtbetaji}{\dot{\tilde{\beta}}_{ji}}
\newcommand{\tcji}{\tilde{c}_{ji}}
\newcommand{\dtcji}{\dot{\tilde{c}}_{ji}}
\newcommand{\tdji}{\tilde{d}_{ji}}
\newcommand{\dtdji}{\dot{\tilde{d}}_{ji}}
\newcommand{\tqji}{\tilde{q}_{ji}}
\newcommand{\dtqji}{\dot{\tilde{q}}_{ji}}
\newcommand{\tlji}{\tilde{\lambda}_{ji}}
\newcommand{\dtlji}{\dot{\tilde{\lambda}}_{ji}}
\newcommand{\tvarphiji}{\tilde{\varphi}_{ji}}
\newcommand{\dtvarphiji}{\dot{\tilde{\varphi}}_{ji}}
\newcommand{\tgji}{\tilde{g}_{ji}}
\newcommand{\dtgji}{\dot{\tilde{g}}_{ji}}


% Node state differences
\newcommand{\xjmi}{x_j-x_i}
\newcommand{\vjmi}{v_j-v_i}
\newcommand{\nxjmi}{\norm{\xjmi}}

% Notation for desired quantities
\newcommand{\xgi}{x_{g,i}}
\newcommand{\xgj}{x_{g,j}}
\newcommand{\betagij}{\beta_{g,ij}}
\newcommand{\dgij}{d_{g,ij}}


==> preamble/graphicsExport.tex <==
% activate externalization of figures
\usetikzlibrary{external}

\tikzexternalize 

%command to insert a Beamer frame from a sketch and externalize with the same name 
\newcommand{\insertsketchframe}[1]{\section{$\mathrm{#1}$}%
\tikzsetnextfilename{#1}%
  \begin{tikzpicture}[scale=0.7]%
    \input{sketch/#1}%
  \end{tikzpicture}%
\endpgfgraphicnamed%
}

%command to insert a Beamer frame from a tikz drawing and externalize with the same name 
\newcommand{\inserttikzframe}[1]{\section{$\mathrm{#1}$}%
\tikzsetnextfilename{#1}%
\input{tikz/#1}%
\endpgfgraphicnamed%
}


==> preamble/math.tex <==
%AMS typesetting
\makeatletter
\@ifpackageloaded{amsmath}{}{%
\usepackage[cmex10]{amsmath}%
}
\makeatother
\usepackage{mathtools}
\usepackage{amssymb,amsfonts}
\makeatletter
\@ifundefined{proof}{%
\usepackage{amsthm}%
}{}
\makeatother

\usepackage{mathtools}

%Common math statements environments
\makeatletter
\@ifundefined{theorem}{
\newtheorem{theorem}{Theorem}
\newtheorem{corollary}{Corollary}
\newtheorem{proposition}{Proposition}
\newtheorem{lemma}{Lemma}
\newtheorem{remark}{Remark}
\newtheorem{fact}{Fact}
}{}
  %SIAM article classes give their own Definition and Remark environments
\@ifundefined{definition}{
  \newtheorem{definition}{Definition}
}
% \@ifundefined{remark}{
%   \newtheorem{remark}{Remark}
% }
\makeatother
\newtheorem{problem}{Problem}
\newtheorem{assumption}{Assumption}
\newtheorem{property}{Property}
\newcommand{\rmss}[1]{_{\textrm{#1}}}

%%% Local Variables: 
%%% mode: latex
%%% End: 


==> preamble/preambleHelp.tex <==
\section*{Markup and commenting commands}
Use the command \var{\textbackslash newcommenter\{cname\}\{color\}} to enable the following commands (substitute \var{cname} with your pseudonim of choice, e.g., \var{rtron}, and \var{color} with a color name supported by the \var{xcolor} package):
\begin{itemize}
\item \var{\textbackslash cname\{comment\}}: typeset a colored comment labeled with the pseudonim.
\item \var{\textbackslash atcname}: use this to refer to another commenter.
\item \var{\textbackslash cnamehl\{comment\}\{text\}}: use this to highligth a portion of the text and comment on it.
\end{itemize}
Examples after using \var{\textbackslash newcommenter\{rtron\}\{Green3\}}:
\begin{itemize}
\item \var{\textbackslash rtron\{Ignore this comment\}} produces \rtron{Ignore this comment}.
\item \var{\textbackslash atrtron} produces \atrtron.
\item \var{\textbackslash rtronhl\{Sentence is obvious\}\{The sky is blue\}} produces \rtronhl{Sentence is obvious}{The sky is blue}
\end{itemize}

Use the command \var{\textbackslash sout} to strike out text.

==> preamble/reviewDraft.tex <==
\usepackage{background}
\backgroundsetup{contents={%
    \begin{tikzpicture}[overlay,font=\sffamily]
      \newcommand{\scaletop}{-.68in}
      \newcommand{\scalepitch}{1.15em}
      \newcommand{\scaleoffset}{.5in}
      \foreach \x in {1,...,60}{
        \node at ($(current page.north west)+(\scaleoffset,\scaletop-\scalepitch*\x)$) {\pgfmathparse{int((\value{page}-1)*200+\x)}\pgfmathresult};
        \node at ($(current page.north east)+(-\scaleoffset,\scaletop-\scalepitch*\x)$) {\pgfmathparse{int((\value{page}-1)*200+100+\x)}\pgfmathresult};
      }
      \node at ($(current page.south)+(0,.5in)$) {*** For Review Only ***};
    \end{tikzpicture}
  },color=blue,scale=1,angle=0}

\author{\textcolor{blue}{\sffamily Author Names Omitted for Anonymous Review}}
\renewcommand{\author}[1]{}


==> preamble/roboticsHelp.tex <==
This file introduces commands for drawing axes and cameras.

\begin{itemize}
\item \var{ax[label][opts]\{refid\}\{x\}\{y\}\{rot\}} Draws a pair of 2-D axes. \var{refid} can be the used to put labels and third axes.
\item \var{axup[label_rotation]\{refid\}\{label\}\{rot\}}
\item \var{axlabels\{refid\}\{label1\}\{label2\}}
\item \var{camera[label]\{refid\}\{x\}\{y\}\{rot\}}
\item \var{gpoint\{coordinates\}\{label\}\{rot\}}
\end{itemize}

